Constructing a Weak Memory Model

Weak memory models are a consequence of the desire on part of architects to preserve all the uniprocessor optimizations while building a shared memory multiprocessor. The efforts to formalize weak memory models of ARM and POWER over the last decades are mostly empirical -- they try to capture empirically observed behaviors -- and end up providing no insight into the inherent nature of weak memory models. This paper takes a constructive approach to find a common base for weak memory models: we explore what a weak memory would look like if we constructed it with the explicit goal of preserving all the uniprocessor optimizations. We will disallow some optimizations which break a programmer's intuition in highly unexpected ways. The constructed model, which we call General Atomic Memory Model (GAM), allows all four load/store reorderings. We give the construction procedure of GAM, and provide insights which are used to define its operational and axiomatic semantics. Though no attempt is made to match GAM to any existing weak memory model, we show by simulation that GAM has comparable performance with other models. No deep knowledge of memory models is needed to read this paper.

==> related_work.tex <==
\section{Related Work}\label{sec:related}
%Out-of-thin-air~\cite{Boehm:2014:OGA:2618128.2618134}.

\newcommand{\etal}{et al.}
\newcommand{\etc}{etc.}

Latest papers:

\mycomment{cited} Sinclair \etal{} \cite{SinclairRats} provide a taxonomy of the different kinds
of synchronization patterns seen in multithreaded code. Based on the different
patterns, they relax the standard DRF requirements and define a DRF-relaxed memory
model, which encompasses all the software patterns they discuss in the paper.

\mycomment{cited} Ros \etal{} \cite{RosTso} specify a clever scheme using out-of-order committing processors, where the cache coherence protocol is modified slightly to implement TSO while allowing loads to be committed out-of-order by the processor.

\mycomment{cited} Shin \etal{} \cite{ShinPersistent} show that speculatively executing non-store operations after persistent fences is necessary to improve performance, and traditional processor-state checkpointing is sufficient to roll back because of issues due to persistent memory.

\mycomment{cited} Kolli \etal{} \cite{KolliLanguage} introduce constructs in the C/C++ language for specifying read, write and barrier operations for persistent memory. This is essentially a specification of a relaxed memory model for persistent memory, while \cite{JoshiPersist, NalliPersistence} define a barrier-only consistency model for persistent accesses.

\mycomment{cited} Alvarez \etal{} \cite{AlvarezCoherence} propose a technique to expose scratchpad memory to programmers, with the aim of making compilation into such a memory system containing scratchpad memories feasible. The result of adding scratchpad memories weakens the memory model -- the programmer has to rely on acquire-release-like synchronization for correct execution.

\mycomment{cited} Alvarez \etal{} \cite{AlvarezRuntime} propose a runtime mechanism to enable scratchpad memories in architectures which are transparent to the programmer, i.e., the mechanism manages scratchpad memory access using a runtime system without changing the memory model.

\mycomment{cited} The check-series of work \cite{ManerkarCCICheck, CarolineTricheck, LustigCoat} provide several tools to test if a particular coherence protocol combines with a particular processor's pipelines and memory hierarchy to enforce the requirements of a given consistency model, for given litmus tests.

\mycomment{cited} Zhang \etal{} \cite{ZhangCoup} provided mechanism to optimize commutative operations in caches without affecting the memory consistency model.

\mycomment{cited} Choi \etal{} \cite{ChoiDenovo} proposed the DeNovo cache coherence protocol, which is a software supported coherence protocol using reader-initiated invalidations and relying on data-race-free program execution for correctness. They showed that the performance is on par with conventional cache coherence protocols while reducing the hardware complexity tremendously.
Sung and Adve \cite{SungDenovo} extended the Denovo protocol to support arbitrary synchronization patterns, not just patterns which protect critical sections using locks. They combine the reader-initiated invalidation of Denovo with writer-initiated invalidation used in conventional protocols to improve performance over Denovo, while ensuring sequentially consistent executions of data-race-free programs.
Sinclair \etal{} \cite{SinclairSimple} show that the DeNovo cache coherence protocol can be implemented efficiently in GPUs, without the need for complicated heterogeneous-race-free (HRF) consistency model.

\mycomment{cited} Singh \etal{} \cite{SinghGpu} and Ren \etal{} \cite{RenGpu} show that enforcing SC/TSO consistency in GPUs does not lose performance as previously thought.

\mycomment{cited} Perais \etal{} \cite{PeraisPredictor} proposed a new value prediction technique that would improve performance considerably. But, it would violate the memory consistency model, including GAM, which enforces ordering for dependent loads.

\mycomment{cited} Kurian \etal{} \cite{Kurian} proposed a mechanism based on timestamps to impose TSO consistency while enabling reordering of memory requests in the cache hierarchy. Xiangyao \etal{} \cite{XiangyaoTardis1, XiangyaoTardis2} cleans up the timestamp-based mechanism and adds support to implement a wider range of consistency models.


\mycomment{cited} Zhang \etal{} \cite{ZhangWmm} propose a new weak memory model using \emph{instantaneous instruction execution}, i.e., the model does not contain a reorder buffer. Instead, all the instruction reorderings, except load-to-store reordering is mimicked by the clever use of invalidation and store buffers.

\mycomment{cited} Alglave \etal{} \cite{AlglaveGpu} specified a consistency model for NVidia GPUs in the HERD notation, and debunked a lot of misconceptions about the behavior of NVidia GPUs (i.e., what possible behaviors are exhibited by programs running on GPUs).

\mycomment{cited} Orr \etal{} \cite{OrrScoped} propose an extension to scoped synchronization of Heterogeneous System Architecture (HSA) memory model for GPUs, adding remote-scope promotion as opposed to static scopes as advocated in HSA. 

\mycomment{cited} Morrison and Afek \cite{MorrisonAfek} introduce a new consistency model called Temporally Bounding TSO which avoids the need for fences on TSO by relying on a bound in the time it takes to drain the store buffer into the memory hierarchy.





\begin{comment}
Lamport's paper on SC \cite{lamport1979make} is probably the first formal
definition, both axiomatic and operational, of a memory model. In the nineties,
three different weak memory models were defined axiomatically for SUN's Sparc
processors: TSO, PSO and RMO~\cite{sparc1992sparcv8,weaver1994sparc}. A weak
memory model for DEC Alpha was also specified axiomatically in the same time
frame~\cite{alpha1998}.  Until a decade ago, however, there was no effort to
specify weak memory models operationally or match axiomatic specifications to
operational models. In this context, papers by Sarkar \etal
\cite{Sarkar:2009:SXM:1594834.1480929}, Sewell \etal \cite{sewell2010x86} and
Owens \etal{} \cite{owens2009better} are very important because they showed
that the axiomatic specification of TSO is exactly equivalent to an operational
model using store buffers connected to I2E processors and atomic memory.

Until recently, weak memory models have not been defined prior to ISA
implementation and have been documented by manufacturers only in an ad hoc
manner using a combination of natural language and litmus tests.  Not
surprisingly, such ``definitions'' have had to be revised as implementations
have changed, revealing new corner cases of behaviors.  Over the last decade,
several studies have been performed, mostly by academic researchers, to
determine the allowed and disallowed behavior of several commercial
microprocessors, with the goal of creating formal models to explain the
observed behaviors.  These studies have been done on real machines by running
billions of instructions and recording the observations (just like studying any
natural phenomenon).  Then, with extra inputs from hardware designers, a model
is constructed that tries to satisfy all these observations.  For example,
Sarkar \etal{} specified an operational model for POWER
\cite{sarkar2011understanding, sarkar2012synchronising}, using a non-atomic
memory.  Later, Mador-Haim \etal{} \cite{mador2012axiomatic} developed an
axiomatic model for POWER and proved that it matches the earlier operational
model.  Alglave \etal{} \cite{alglave2009semantics, Alglave2011,
alglave2012formal, alglave2014herding, alglave2013software} give axiomatic
specifications for ARMv7 and POWER using the Herd framework; Flur \etal{}
\cite{flur2016modelling} give operational specification for ARMv8.

However, there has been some dispute if the operational model of POWER models
actual POWER processors accurately \cite{alglave2014herding}. We attribute the
reason for the potential errors to be the inherent complexity of the
operational model because of the use of non-atomic memory.  Alglave models are
not sufficiently grounded in operational models and face the problem of being
too liberal. The model may admit behaviors which cannot be observed in any
implementation. Such models can also lead to insertion of unnecessary fences in
a program.  We think it is important to have matching operational and axiomatic
models.

Researchers have also proposed several other consistency models: Processor
Consistency~\cite{goodman1991cache}, Weak Consistency~\cite{dubois1986memory},
RC~\cite{gharachorloo1990memory}, CRF~\cite{shen1999commit}, Instruction
Reordering + Store Atomicity~\cite{arvind2006memory}.  The tutorials by Adve
\etal{} \cite{adve1996shared} and by Maranget \etal{}
\cite{maranget2012tutorial} provide relationships among some of these models.

Researchers have also proposed architectural mechanisms for implementing SC
\cite{lamport1979make} efficiently
\cite{gharachorloo1991two,ranganathan1997using,guiady1999sc+,gniady2002speculative,ceze2007bulksc,wenisch2007mechanisms,blundell2009invisifence,singh2012end,lin2012efficient,gope2014atomic}.
Several of these architectural mechanisms are interesting in their own right
and applicable to reducing power consumption, however, so far commercial
processor vendors have shown little interest in adopting stricter memory
models.


Recently, there is a splurge of activity in trying to specify semantics of
concurrent languages: C/C++
\cite{c++n4527,boehm2008foundations,batty2011mathematizing,Batty:2016:OSA:2914770.2837637,Kang:2015:FCM:2737924.2738005},
Java \cite{manson2005java,cenciarelli2007java, maessen2000improving}.  These
models are specified axiomatically, and allow load-store reordering.  For C++,
there has been work to specify an equivalent operational model
\cite{operationalC++}.
\end{comment}

%% The check series of work presents a methodology to test if a specific
%% microarchitectural specification (which is conceptually similar to an
%% operational model) adheres to an axiomatic memory model specification,
%% for a set of litmus tests \cite{}. They have recently extended their
%% methodology to include RTL verification \cite{RTLCheck} (maybe a CoRR
%% version is more appropriate since ISCA is too far off?).

%% Recently, Lustig \etal{} have used Memory Ordering Specification
%% Tables (MOSTs) to describe memory models, and proposed a hardware
%% scheme to dynamically convert programs across memory models described
%% in MOSTs \cite{lustig2015armor}.  MOST specifies the ordering strength
%% (e.g., locally ordered, multicopy atomic) of two instructions from
%% the same processor under different conditions (e.g., data dependency,
%% control dependency).  Our work is orthogonal in that we propose new
%% memory models with equivalent operational and axiomatic definitions,
%% that are proved manually.

%% Adve and Hill defined Data-Race-Free-0 (DRF0), a class of programs where shared variables are protected by locks, and proposed that DRF0 programs should behave as SC \cite{adve1990weak}.
%% However, architectural memory models must also define the behaviors of non-DRF0 programs.

%% Arvind and Maessen have specified the conditions for preserving store
%% atomicity in program execution when instructions can be reordered
%% \cite{arvind2006memory}.  In contrast, GAM do not insist on store
%% atomicity at the program level.






